The Astrophysics of Nanohertz Gravitational Waves

Pulsar timing array (PTA) collaborations in North America, Australia, and Europe, have been exploiting the exquisite timing precision of millisecond pulsars over decades of observations to search for correlated timing deviations induced by gravitational waves (GWs). PTAs are sensitive to the frequency band ranging just below 1 nanohertz to a few tens of microhertz. The discovery space of this band is potentially rich with populations of inspiraling supermassive black-holes binaries, decaying cosmic string networks, relic post-inflation GWs, and even non-GW imprints of axionic dark matter. This article aims to provide an understanding of the exciting open science questions in cosmology, galaxy evolution, and fundamental physics that will be addressed by the detection and study of GWs through PTAs. The focus of the article is on providing an understanding of the mechanisms by which PTAs can address specific questions in these fields, and to outline some of the subtleties and difficulties in each case. The material included is weighted most heavily towards the questions which we expect will be answered in the near-term with PTAs; however, we have made efforts to include most currently anticipated applications of nanohertz GWs.

==> sec_smbh_galaxymergers.tex <==

Galaxies are observed to merge and contain SMBHs at their nuclei, but large uncertainties exist in the galaxy merger rate and the SMBH mass distribution.  While the spectral index of the GW background spectrum is determined by the rate at which binaries harden, the normalization (amplitude) is determined by the distribution of merger rates and masses. 
After the first detections of the GW background, PTA will be able to provide some constraints on the degree of anisotropy in the source distribution which may provide independent constraints on these uncertain parameters.

A growing number of angularly-resolvable, dual-AGN systems have been identified across the electromagnetic spectrum in surveys from the X-ray \fixme{(comerford+...)}, optical \fixme{(greene+...)}, and radio \fixme{(Rodriguez+2007, Burke-Spolaor+...)}.  Most telescopes cannot resolve sub-parsec scales in galaxies making the identification of resolvable close-binary systems intractable.  Numerous alternative methods are being employed to infer the presence of an MBH binary based on observations of only a single AGN.  Two commonly used methods are 1) photometric variability \fixme{Graham+2015, charisi+2016}, where there is a periodic modulation of AGN brightness, and 2) spectroscopic redshifts indicating a large velocity offset between AGN components.

If MBH-binaries merge effectively, then there should be a strong signal in the PTA band.  Otherwise, there should be a large number of `stalled' binary systems which could be observed electromagnetically or through their influence on the local stellar population (e.g. TDE).

